Designing Equitable Transit Networks

Public transit is an essential infrastructure enabling access to employment, healthcare, education, and recreational facilities. While accessibility to transit is important in general, some sections of the population depend critically on transit. However, existing public transit is often not designed equitably, and often, equity is only considered as an additional objective post hoc, which hampers systemic changes. We present a formulation for transit network design that considers different notions of equity and welfare explicitly. We study the interaction between network design and various concepts of equity and present trade-offs and results based on real-world data from a large metropolitan area in the United States of America.

==> plots/BarPlots_chatt.tex <==
\begin{figure}[ht]
\centering
%\begin{subfigure}[b]{.5\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/demand.tex}}
%\caption{Chattanooga, Hamilton County, TN}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.5\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/franklin/demand.tex}}
% \caption{Franklin, Williamson County, TN}
% \end{subfigure}
\caption{Distribution of Demand across Priority Groups}
\label{fig:Demand}
\end{figure}

==> plots/Base_Service_Frank.tex <==
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/difference/MaxMinEP_UEP.tex}}
\caption{Rawlsian Equal Priorities}
\label{r_ep_f}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/difference/MaxMinP_UEP.tex}}
\caption{Rawlsian Unequal Priorities}
\label{r_p_f}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/Utilitarian/service_EP.tex}}
\caption{Percentage of People Served} 
\label{u_ep_f}
\end{subfigure}
\caption{(\subref{r_ep_f}) (\subref{r_p_f}) The gain in average utility compared to a utilitarian baseline, and (\subref{u_ep_f}) Percentage of people served by the utilitarian baseline in Franklin, Williamson County, TN.}
\label{fig:ServeBase_Frank}
\end{figure*}

==> plots/Chatt_LC.tex <==
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.1$: Chattanooga, Hamilton County, TN}
\label{fig:ChattLC1}
\end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.3/EP.tex}}
% \caption{Equal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.3/P.tex}}
% \caption{Unequal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.3/difference.tex}}
% \caption{Utility Gain} 
% \end{subfigure}
% \caption{Average Utility and Gain based on the Linear Combination Formulation, $gamma = $0.3: Chattanooga, Hamilton County, TN}
% \label{fig:ChattLC3}
% \end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.5$: Chattanooga, Hamilton County, TN}
\label{fig:ChattLC5}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.7$: Chattanooga, Hamilton County, TN}
\label{fig:ChattLC7}
\end{figure*}

==> plots/Frank_LC.tex <==
%lc 0.1
\begin{figure*}[htbp]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.1/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.1/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.1/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.1$: Franklin, Williamson County, TN}
\label{fig:FrankLC1}
\end{figure*}

%lc 0.5
\begin{figure*}[htbp]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.5/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.5/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.5/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.5$: Franklin, Williamson County, TN}
\label{fig:FrankLC5}
\end{figure*}

%lc 0.7
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.7/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.7/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/LinearCombo/gamma0.7/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Linear Combination Formulation, $\gamma = 0.7$: Franklin, Williamson County, TN}
\label{fig:FrankLC7}
\end{figure*}

==> plots/Frank_main.tex <==
\begin{figure*}[htbp]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/Utilitarian/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/Utilitarian/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/Utilitarian/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Utilitarian Formulation: Franklin, Williamson County, TN}
\label{fig:UtilitarianFrank}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/MaxMin/EP.tex}}
\caption{Equal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/MaxMin/P.tex}}
\caption{Unequal Priorities}
\end{subfigure}\hfill
\begin{subfigure}[b]{.33\textwidth}
\resizebox{1\columnwidth}{!}{
\input{plots/line_plot/franklin/center/MaxMin/difference.tex}}
\caption{Utility Gain} 
\end{subfigure}
\caption{Average Utility and Gain based on the Rawlsian Formulation: Franklin, Williamson County, TN}
\label{fig:MaxMinFrank}
\end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/Utilitarian/EP.tex}}
% \caption{Equal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/Utilitarian/P.tex}}
% \caption{Unequal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/Utilitarian/difference.tex}}
% \caption{Utility Gain} 
% \end{subfigure}
% \caption{Average Utility and Gain based on the Utilitarian Formulation: Chattanooga, Hamilton County, TN}
% \label{fig:Utilitarian}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/MaxMin/EP.tex}}
% \caption{Equal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/MaxMin/P.tex}}
% \caption{Unequal Priorities}
% \end{subfigure}\hfill
% \begin{subfigure}[b]{.33\textwidth}
% \resizebox{1\columnwidth}{!}{
% \input{plots/line_plot/chattanooga/center/MaxMin/difference.tex}}
% \caption{Utility Gain} 
% \end{subfigure}
% \caption{Average Utility and Gain based on the Rawlsian Formulation: Chattanooga, Hamilton County, TN}
% \label{fig:MaxMin}
% \end{figure*}

==> plots/Plots_Chatt_Center.tex <==
\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/Utilitarian/EP.tex}}
        \caption{Chattanooga Utilitarian Homogeneous Priorities}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/Utilitarian/P.tex}}
        \caption{Chattanooga Utilitarian Heterogeneous Priorities}
    \end{subfigure}%
\end{figure}
\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/MaxMin/EP.tex}}
        \caption{Chattanooga MaxMin Homogeneous Priorities}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/MaxMin/P.tex}}
        \caption{Chattanooga MaxMin Heterogeneous Priorities}
    \end{subfigure}%
\end{figure}
\begin{figure}[ht]
\centering
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/Utilitarian/service_EP.tex}}
        \caption{Chattanooga Utilitarian Homogeneous Priorities}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{1\linewidth}
        \resizebox{0.98\columnwidth}{!}{\input{plots/line_plot/chattanooga/center/Utilitarian/service_P.tex}}
        \caption{Chattanooga Utilitarian Heterogeneous Priorities}
    \end{subfigure}%
\end{figure}
\begin{figure}[ht]
\centering
{\input{plots/line_plot/chattanooga/demand.tex}}
\caption{Percentage of Total Cumulative Demand per Priority Group}
\end{figure}

\begin{figure}[ht]
\centering
{\input{plots/line_plot/chattanooga/center/Utilitarian/difference.tex}}
\caption{Utility Gained with Utilitarian}
\end{figure}

\begin{figure}[ht]
\centering
{\input{plots/line_plot/chattanooga/center/MaxMin/difference.tex}}
\caption{Utility Gained with MaxMin}
\end{figure}

\begin{figure}[ht]
\centering
{\input{plots/line_plot/chattanooga/center/difference/MaxMinEP_UtilEP.tex}}
\caption{Difference in Average Utility MaxMin EP and Utilitarian EP}
\end{figure}

\begin{figure}[ht]
\centering
{\input{plots/line_plot/chattanooga/center/difference/MaxMinP_UtilEP.tex}}
\caption{Difference in Average Utility MaxMin P and Utilitarian EP}
\end{figure}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_EP_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_EP_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_EP_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_EP_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_EP_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_P_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_P_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_P_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_P_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_P_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.1/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.19, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_chatt_lc_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_chatt_lc_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_chatt_lc_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_chatt_lc_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_chatt_lc_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.3/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_EP_3.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_EP_3.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_EP_3.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_EP_3.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_EP_3.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.3/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
% \addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_P_3.csv};

% \addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_P_3.csv};

% \addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_P_3.csv};

% \addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_P_3.csv};

% \addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_P_3.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_EP_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_EP_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_EP_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_EP_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_EP_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_P_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_P_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_P_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_P_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_P_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.5/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.19, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_chatt_lc_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_chatt_lc_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_chatt_lc_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_chatt_lc_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_chatt_lc_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_EP_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_EP_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_EP_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_EP_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_EP_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.76, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/chatt_center_lc_P_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/chatt_center_lc_P_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/chatt_center_lc_P_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/chatt_center_lc_P_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/chatt_center_lc_P_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/LinearCombo/gamma0.7/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.19, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_chatt_lc_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_chatt_lc_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_chatt_lc_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_chatt_lc_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_chatt_lc_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/chattanooga/center/Utilitarian/service_P.tex <==
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin=0.955,
ylabel={Percentage of Demand Served},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/percentageServed_U_P.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/percentageServed_U_P.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/percentageServed_U_P.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/percentageServed_U_P.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/percentageServed_U_P.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}

==> plots/line_plot/demand.tex <==
\begin{adjustbox}{totalheight=0.075in}
\begin{tikzpicture}
\begin{axis}
[ 
ybar,
ymin = 0, ymax=1.0,
xtick = data,
  legend image code/.code={%
                    \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.6cm,0.1cm);
                },  
symbolic x coords={Group 1, Group 2, Group 3, Group 4, Group 5},
tick label style={font=\footnotesize}, 
ylabel=Fraction of Demand,
xlabel=Priority Group,
 nodes near coords,
    nodes near coords style={anchor=east,rotate=-90,inner xsep=1pt}
]
\addplot[ybar,fill, color=vermillion] table [x, y=d, col sep=comma] {csvs/demand_hist.csv};
\addplot[ybar,fill, color=blue] table [x, y=d, col sep=comma] {csvs/demand_hist_frank.csv};
\legend {Chattanooga, Franklin};

\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.1/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.7, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_EP_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_EP_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_EP_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_EP_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.1/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.7, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_P_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.1/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.39, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_frank_lc_1.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_frank_lc_1.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_frank_lc_1.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_frank_lc_1.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_frank_lc_1.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.5/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.55, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_EP_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_EP_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_EP_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_EP_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.5/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.55, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_P_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.5/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.39, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_frank_lc_5.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_frank_lc_5.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_frank_lc_5.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_frank_lc_5.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_frank_lc_5.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.7/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.53, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_EP_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_EP_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_EP_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_EP_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_EP_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.7/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.53, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_lc_P_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_lc_P_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_lc_P_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_lc_P_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_lc_P_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/LinearCombo/gamma0.7/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.35, ymax = 0.15,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_frank_lc_7.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_frank_lc_7.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_frank_lc_7.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_frank_lc_7.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_frank_lc_7.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/MaxMin/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.7, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_MaxMin_EP.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_MaxMin_EP.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_MaxMin_EP.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_MaxMin_EP.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_MaxMin_EP.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/MaxMin/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.7, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_MaxMin_P.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_MaxMin_P.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_MaxMin_P.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_MaxMin_P.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_MaxMin_P.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/MaxMin/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.19, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_frank_mm.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_frank_mm.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_frank_mm.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_frank_mm.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_frank_mm.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/Utilitarian/EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.56, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_Utilitarian_EP.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_Utilitarian_EP.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_Utilitarian_EP.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_Utilitarian_EP.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_Utilitarian_EP.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/Utilitarian/P.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = 0.56, ymax = 1.025,
ylabel={Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/frank_center_Utilitarian_P.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/frank_center_Utilitarian_P.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/frank_center_Utilitarian_P.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/frank_center_Utilitarian_P.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/frank_center_Utilitarian_P.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/Utilitarian/difference.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.19, ymax = 0.17,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/difference_u_frank.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/difference_u_frank.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/difference_u_frank.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/difference_u_frank.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/difference_u_frank.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/Utilitarian/service_EP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.04)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin=0.825,
ylabel={Percentage of Demand Served},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/percentageServed_U_EP_frank.csv};
\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/percentageServed_U_EP_frank.csv};
\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/percentageServed_U_EP_frank.csv};
\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/percentageServed_U_EP_frank.csv};
\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/percentageServed_U_EP_frank.csv};
\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/difference/MaxMinEP_UEP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.25, ymax = 0.25,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/MaxMinEP_UEP_frank.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/MaxMinEP_UEP_frank.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/MaxMinEP_UEP_frank.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/MaxMinEP_UEP_frank.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/MaxMinEP_UEP_frank.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/center/difference/MaxMinP_UEP.tex <==
\begin{adjustbox}{totalheight=0.2in}
\begin{tikzpicture}
\begin{axis}[
legend style={
            font=\tiny,
            at={(0.8,.6)},
            anchor=south,
            % legend rows=-5
        },
xlabel={Budget},
grid=both,
    grid style={line width=.1pt, draw=gray!10},
     minor tick num=5,
    major grid style={line width=.2pt,draw=gray!50},
% x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
ymin = -0.25, ymax = 0.25,
ylabel={Difference in Average Utility},
]
\addplot [color=SkyBlue] table [x=normal, y=p_1, col sep=comma] {csvs/MaxMinP_UEP_frank.csv};

\addplot [color=orange] table [x=normal, y=p_2, col sep=comma] {csvs/MaxMinP_UEP_frank.csv};

\addplot [color=BlueGreen] table [x=normal, y=p_3, col sep=comma] {csvs/MaxMinP_UEP_frank.csv};

\addplot [color=black] table [x=normal, y=p_4, col sep=comma] {csvs/MaxMinP_UEP_frank.csv};

\addplot [color=vermillion] table [x=normal, y=p_5, col sep=comma] {csvs/MaxMinP_UEP_frank.csv};

\legend{Priority Group 1, Priority Group 2, Priority Group 3, Priority Group 4, Priority Group 5}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

==> plots/line_plot/franklin/demand.tex <==
\begin{adjustbox}{totalheight=0.075in}
\begin{tikzpicture}
\begin{axis}
[ 
xtick = data,
xticklabels={Group 1, Group 2, Group 3, Group 4, Group 5},
tick label style={font=\footnotesize}, 
ylabel=Percentage of Demand,
xlabel=Priority Group,
ymin = 0, ymax=1.0,
]
\addplot[ybar,fill, color=vermillion] table [x, y=d, col sep=comma] {csvs/demand_hist_frank.csv};
\end{axis}
\end{tikzpicture}
\end{adjustbox}
